Getting ViT in Shape: Scaling Laws for Compute-Optimal Model Design

Scaling laws have been recently employed to derive compute-optimal model size (number of parameters) for a given compute duration. We advance and refine such methods to infer compute-optimal model shapes, such as width and depth, and successfully implement this in vision transformers. Our shape-optimized vision transformer, SoViT, achieves results competitive with models that exceed twice its size, despite being pre-trained with an equivalent amount of compute. For example, SoViT-400m/14 achieves 90.3% fine-tuning accuracy on ILSRCV2012, surpassing the much larger ViT-g/14 and approaching ViT-G/14 under identical settings, with also less than half the inference cost. We conduct a thorough evaluation across multiple tasks, such as image classification, captioning, VQA and zero-shot transfer, demonstrating the effectiveness of our model across a broad range of domains and identifying limitations. Overall, our findings challenge the prevailing approach of blindly scaling up vision models and pave a path for a more informed scaling.

==> tabs/i1k-linear-transpose.tex <==
\begin{wraptable}{r}{0.5\linewidth}
  \setlength{\tabcolsep}{5pt}
  \setlength{\extrarowheight}{5pt}
  \renewcommand{\arraystretch}{0.8}
  \centering
  \vspace{0em}
  \begin{tabulary}{1.0\linewidth}{LCCC}
    \toprule
\bf{I'Net} & \bf{ViT-L/16} & \bf{SoViT-400m/14} & \bf{ViT-g/14} \\ 
    \midrule
Val & 86.7 & 88.2 & \bf{88.4} \\ 
-ReaL & 90.0 & \bf{90.3} & 90.2 \\ 
-v2 & 78.5 & 80.6 & \bf{80.8} \\ 
-R & 88.9 & 89.0 & \bf{90.3} \\ 
-A & 67.8 & 76.4 & \bf{76.6} \\ 
ObjNet & 63.5 & \bf{68.7} & 67.7 \\ 
    \bottomrule
  \end{tabulary}
  \caption{Blabla}\label{tbl:i1k_linear}
  \vspace{-1em}
\end{wraptable}



